AI Challenges in Human-Robot Cognitive Teaming

Among the many anticipated roles for robots in the future is that of being a human teammate. Aside from all the technological hurdles that have to be overcome with respect to hardware and control to make robots fit to work with humans, the added complication here is that humans have many conscious and subconscious expectations of their teammates - indeed, we argue that teaming is mostly a cognitive rather than physical coordination activity. This introduces new challenges for the AI and robotics community and requires fundamental changes to the traditional approach to the design of autonomy. With this in mind, we propose an update to the classical view of the intelligent agent architecture, highlighting the requirements for mental modeling of the human in the deliberative process of the autonomous agent. In this article, we outline briefly the recent efforts of ours, and others in the community, towards developing cognitive teammates along these guidelines.

==> sections/abstract.tex <==
\begin{abstract}

Among the many anticipated roles for robots in future is that of being a
human teammate.  Aside from all the technological hurdles that
have to be overcome on the hardware and control sides to make robots
fit for work with humans, the added complication here is that
humans have many conscious and subconscious expectations of their
teammates -- indeed, teaming is mostly a {\em cognitive} rather than {\em 
physical} coordination activity.  This focus on cognitive
coordination, however, introduces new challenges for the robotics community that
require fundamental changes to the traditional view of autonomous agents.

In this paper, we provide an analysis of the differences between
traditional autonomous robots and robots that team with humans,
identifying the necessary teaming capabilities that are largely
missing from current robotic systems.  
We then focus on the important
challenges that are unique and of particular importance to human-robot teaming, 
especially from the point of view of the deliberative process of the autonomous agent,
and sketch potential ways to address them.

\end{abstract}


==> sections/challenges.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Challenges - Multi Model Planning} % (fold)
\label{sec:challenges}

These desired capabilities for teaming robots reflected in the new updated view of the cognitive agent
architecture present several challenges for the design of robotic teammates which are yet to be addressed or has at least seen research in the nascent state of late.
At the core of these issues is the need for an autonomous agent to consider not only its own model but also the human teammate's mental model as well in its deliberative process.  
In the following discussion, we will outline a few such directions under the umbrella of Multi-Model Planning \cite{explain, exply} - we will first outline two processes by which an autonomous agent can deal with such multiple models, and follow up with a discussion on work aimed at learning and evaluating such models. One of the crucial aspects of the cognitive teaming paradigm is the need to be able to deal with the Human Mental Model (HuMM) in addition to the robot's own model - this situation is shown in Fig. \ref{fig:mmp} where the HuMM consists of both the human's intentions / capabilities ($M_H$) as well as her expectations ($M^H_R$) of the robot teammate which has its own model ($M_R$).
The autonomous agent, in such a setting, can adapt its own plans to be closer to the human's expectations or reconcile any model differences in course of interactions. The former, referred to as ``human-aware planning'', enables a robot to become a social agent and while the latter in the form of model-reconciliation builds trust and teamwork over time.

\begin{figure}[tbp]
\centering
\includegraphics[width=\columnwidth]{figure/hap}
\caption{The expanding scope of human-aware planning (HAP) to account for the human model (HuM) and the human mental model (HuMM).}
\label{fig:hap}
\end{figure}

\begin{figure}[tbp]
\centering
\includegraphics[width=\columnwidth]{figure/mmp}
\caption{Explanation generation \cite{explain} via the model reconciliation process to make optimal plans in the robot's model also optimal, and hence, explicable in the updated human model and explicable plan generation \cite{exply} by sacrificing optimality in the robot's model in the Multi-Model Planning (MMP) setting.}
\label{fig:mmp}
\end{figure}

\subsection{Human Aware Planning \& Explicable Behavior}

Most traditional approaches to planning focus on one-shot planning in
closed worlds given complete domain models.  While even this problem
is quite challenging, and significant strides have been made in taming
its combinatorics, planners for robots in human-robot teaming
scenarios require the ability to be {\it human-aware}.  Human-aware
planning is especially challenging since it must not only consider human physical state,
 but also their mental state as we discussed, which are inherently incomplete.  
 Furthermore, different human models capture different
aspects of the human (e.g., capabilities \cite{yu-aamas}, intentions \cite{6942970} and emotions \cite{scheutzschermerhorn09handbook})
which are closely inter-related, and it is not clear how they can be combined.  
In the robotics and automated planning communities, there has been some work
on human-aware planning, from the aspect of both path planning
\cite{cnrs,kuderer} and task planning \cite{tist, tathagata-serendipity-iros, tathagata-conflict-aamas, mipc,Chakraborti2016AFF} with the intention of making robot plans more socially acceptable (e.g., resolving conflicts with the plans of fellow humans) and reducing prior communication for coordination.  
However, most of these approaches assume that human models are provided, and they are accurate and complete.

A robot which is socially aware can adapt its own planning process in order to be explicable from the human's perspective (i.e. plan or act considering the robot's approximation of the human's model of itself, instead of just its own model).
There exists some recent work on planning while 
considering the human expectation both while computing trajectories \cite{Dragan-RSS-13,Dragan2015a,Dragan2015b} as well as longer term task plans \cite{grandpa,zhang2016plan,exply,exp-anagha}.
The latter line of work introduces
a plan explicability measure \cite{zhang2016plan} learned approximately from labeled plan traces as a proxy to the human model.
%explicitly
This captures the human expectation of the robot, which can be
used by agents to proactively choose, or directly incorporated into
the planning process to generate plans that are more comprehensible 
without affecting the quality too much.
This is, however, only a start in this research direction. 
Performing human-aware planning with incomplete models remains an
important challenge in human-aware planning, especially given that we do not yet 
understand how these different human models interact.

\subsection{Model Reconciliation \& Long-term Teaming}

If the robot were to stick to its own model instead, it can explain away different aspects of its planning and execution process \cite{pat} when required. 
Such explanations must not only make sense of the plan generation process itself \cite{kambhampati1990classification,sohBiaMcIAAAI2011}, but must also make sense from the (robot's understanding of the) human's perspective \cite{explain}.
This is usually an implicit assumption in the explanation generation process; e.g. imagine a teacher explaining to a student - this is done in a manner so that the student can make sense of the information in their model. This is also true in case of human-robot teams, where the human's understanding of the robot may not be accurate.
Such explanations must not only be able to justify failure \cite{goebelbecker2010coming,Herzig:2014:RPT:3006652.3006726,menezes2012planning,eiter2010updating} but also the rationale behind a successful plan in order for the human to be able to reason about the situation and contrast among alternative hypotheses \cite{explain,lombrozo2012explanation,Lombrozo2006464}.
Further, explanations must be communicated at a level understandable to the human \cite{16roman-verbalization,16ijcai-verbalization}.

All these processes are aimed at bringing the robot's model and the human expectation of it closer over continued interactions. 
We have so far only discussed how a robot can maintain the human mental models. 
However, in teaming, this modeling is bi-directional. 
When robots do not have certain information, 
the robot can plan to sense and communicate with the human. 
In cases when the human is suspected to have insufficient
information about the robot, the robot needs to proactively communicate its model
to the human.  
This communication can be, for example, about the
intention, plan, explanations and excuses of behavior \cite{excuses-icaps} for
the robot; communication can involve different modalities such as
visual projection, natural languages, gesture signaling, and a mixture
of them.  
This capability is important for the human and robot to evolve their mental models
to improve teaming in the long term.
Note that the models (i.e., the human actual model and its representation on the robot) are not required to be aligned, 
which is often only applicable for repetitive tasks \cite{Nikolaidis:2013}.
Much existing work on robots
communicating with humans using different modalities can be utilized
\cite{kollaretal10hri, Tellex14askingfor}.  
However, a more critical challenge for the robot is
to compute when, what, and how
to communicate for model adaptation %for long-term teaming.  
- communicating too much information can increase
the cognitive load of the human teammates while communicating too
little can decrease the teaming situation awareness. 

It must also be realized that
many human-robot teaming tasks are not only complex, 
but can also span multiple episodes for an extended period of time. 
In such scenarios, the system's performance is dependent on 
how the teams perform in the current task, 
as well as how they perform in future tasks.  
A prerequisite to consider long-term teaming is to maintain mental states of the agents (e.g., trust)
that influence their interactions, 
and analyze how these states dynamically affect the teaming performance 
and how they evolve over time. 

\vspace{5pt}
\paragraph{\textbf{Remark}} 
Clearly the two approaches discussed above are closely related and the robot will end up having to face with some degree of either problem -- the robot may be unable to use the human's expectation completely (if it is significantly away from the ground truth) in which case explanations become necessary, while the ability to adapt itself reduces the actual need for explanations later on.

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figure/spectrum-fig-tathagata}
\caption{A schematic view of the different classes of incomplete models and the relationships between them in the spectrum of incompleteness \cite{hankz-wv-reg}.}
\label{fig:incomplete}
\end{figure*}

\subsection{Towards HuMMs \& Cognitive Teaming}

Of course, both the previous challenges were built on the premise that the human mental model was available or at least learned so as to facilitate the decision making process with this model in mind. Acquiring of such models, taken for granted among human teammates through centuries of evolution, is perhaps the hardest challenge to be overcome to realize truly cognitive teaming. The difficulty of this problem is exacerbated by the fact that much (specifically, $M^H_R$) of the HuMM cannot be learned from observations directly but only from continued interactions with the human. Further, we emphasize the importance of human factors studies to complement algorithmic development in these fields to ensure that different models of autonomy are evaluated accurately.

\vspace{5pt}
\subsubsection{Learning the Human Mental Model}
%The first challenge in cognitive teaming is for robots to create and maintain models of the human teammates that capture their capabilities, preferences, intentions and etc.  
%This naturally occurs between human teammates as they work collaboratively in the environment.  
These models are inherently partial from the robot's
perspective and must be learnable.  As a result, they are often
subject to a high level of incompleteness.  However, most work on
planning has hitherto focused on complete world
models~\cite{nau-text,geffner-book,rao-aimag}, while most real-world
scenarios, especially when they involve humans, have a critical
defining property that eliminates these standard planning and
problem-solving methods: they are {\em open-ended} in that planning
agents typically do not have sufficient knowledge about all
task-relevant information (e.g., human models) at planning time -- in
other words, the planning models would be incomplete
\cite{Kambhampati07model-liteplanning}.  Despite being incomplete,
such models must support reasoning as well as being improvable from
sensing (which includes explicitly asking the human).  Hence, an
important challenge is to develop representations of approximate and
incomplete models that are easy to learn (for human mental modeling) and can support
planning/decision-making (for anticipating human behavior).

Existing work on incomplete models (Figure \ref{fig:incomplete}) 
differ in the information that is available for model learning, as well
as how planning is performed.  
Some of them start with complete action
models, such as STRIPS, and modify them with
possible precondition/effect annotations to support incompleteness
\cite{tuan-ICAPS-2014,tuan-nips,hankz-mlcbp,Zhuo:2013,hankz-macrops}.
Although these models support principled approaches for robust
planning, they are still quite difficult to learn.  On the other end
of the spectrum, are very shallow models \cite{hankz-wv-reg}
that assume no structured information at all which are used mainly in
short-term planning support.  There are also partial models that are
somewhere in between \cite{yu-aamas}, which has more structured
information while is still easy to learn. 
However, planning under this model is incomplete. 
These prior models only form a starting point of
work in this direction and considerable research effort still remains to be invested 
in the development and analysis of such models.

\vspace{5pt}
\subsubsection{Human-factors Analysis and Evaluation}
%{\bf MS: this section strikes me a repetitive and out-of-place here,
%  as some of these questions should have come earlier; maybe we can
%  move some of the first paragraph to the beginning of this section
%  and removed the rest?}
The analysis of human-human and human-animal teams,
as well as the verification and evaluation of the performance
of developed robotic systems is a challenging but necessary task.  
%While this may seem less obvious, it is an important part of the equation to develop cognitive robotic teammate. 
Although the teamwork literature \cite{cooke2013interactive} has identified characteristics of
effective and ineffective teams,
it is less clear what characteristics are
essential at the individual level to be a good team player. To what extent do lessons from 
human-human studies carry over to the design of autonomy?  
What are the most important behaviors that a teammate must exhibit 
for effective teaming?  For instance, how should we tradeoff closed-loop-communication 
with the development of a good understanding of team
members' intentions and capabilities?  The
challenge here is to understand the relative importance of these aspects
under different contexts and adopt them towards the needs of a cognitive robotic teammate.

In terms of evaluation, 
it is well known that automation can have both
positive and negative effects on human performance.  Fortunately,
there are many theories and findings from the human teaming literature
that are relevant to human-robot teaming.  For instance, we know that
team effectiveness is tied to shared mental models
\cite{Bowers,Mathieu2000}, team situational awareness
\cite{nancy-new}, and interaction \cite{nancy2013}.  
Although it seems only naturally to assume that 
 effective robotic team players will need to have
similar capabilities for understanding their teammates and the situation
and for communicating their actions to teammates,
and there exists work that tried to partly verify this claim \cite{hri, iros-hri},
it still remains to be evaluated more extensively.





%\begin{figure}
%\centering
%{
%    \includegraphics[scale=0.9]{figure/human-human}
%}
%\caption{Virtual testbed of human-robot teaming scenarios.}
%\label{}
%\end{figure}



==> sections/conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}

In this paper, we discussed the challenges in design of autonomous robots 
that are cognizant of the cognitive aspects of working with human teammates.  
We argued that traditional goal-based and
behavior-based agent architectures are insufficient for building robotic teammates.
Starting with the traditional view of a goal-based agent, we expand it
to include a critical missing component: human mental modeling.  We
discussed the various tasks that are involved when such models are
present, along with the challenges that need to be addressed to
achieve these tasks.  We hope that this paper can serve as guidance
for the development of robotic systems that can enable 
more natural teaming with humans.


==> sections/introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}

An increasing number of applications demand that humans and robots
work together.  Although a few of these applications can be handled
through ``teleoperation'', technologies that act in concert with the
humans in a teaming relationship with increasing levels of autonomy
are often desirable if not required.  Even with a sufficiently robust human-robot
interface, robots will still need to exhibit
characteristics common in human-human teams in order to be good team players.
This includes the ability to
recognize the intentions of the human teammates, and to interact in
a way that is comprehensible to them - 
autonomous robots need to understand and adapt to human behavior 
in an efficient manner, much like humans adapt to the
behavior of other humans.

Consider, for example, a search and rescue team where one searcher is in
need of a tool to open a blocked passage way and another searcher upon
watching the first immediately dashes over to provide help with
lifting a heavy pole that could be used to pry open the broken door.
Or take the surgery assistant that proactively picks a gauze to press
down on the bleeding tissue after the surgeon finished making the
incision.  These are two simple, but typical examples of how humans
coordinate their activities in teams, especially experienced teams, often
without the need of explicit communication during coordination.  It is
this type of coordination that contributes to the highly
efficient teaming between humans.

The reason why humans are able to perform these proactive steps and
support others in their goals is the human ability to quickly 
$(1)$ recognize teaming context in terms of the current status of the team 
(i.e., status of the team task and states of the teammates),
$(2)$ anticipate next team behavior under the current context 
to decide the individual subgoals to be achieved for the team, 
and $(3)$ take proper actions to support the advancement of those subgoals
with the consideration of the other teammates.
Within these steps, explicit communication may be used to facilitate the collaboration 
when necessary.

The three steps
above form a tightly coupled integrated loop 
%such that they are intermixed with each other 
during the coordination process, which
allows humans to adapt to changing circumstances and update
their understanding about the current status of the team,
infer about teammate intentions, goals and preferences to predict their behavior 
in the context of the team task,
and act in ways that are consistent with expected teaming behavior. 
Furthermore, this process is constantly evolving for the team during teaming experience. 
Critically, humans will likely expect all of the above capabilities from a robotic
teammate, as otherwise team dynamics will suffer.

As such, the challenge in human-robot teaming is primarily {\em cognitive}, 
rather than physical.
Cognitive teaming allows the robots to adapt more proactively to the 
many conscious and subconscious expectations of their human teammates. 
At the same time, improper design
of such robot autonomy could increase the human's cognitive load, 
leading to the loss of teaming situation awareness, 
misaligned coordination, 
poorly calibrated trust, 
and ultimately slow decision making, deteriorated teaming performance, 
and even safety risks to the humans. 
As designers of robotic control architectures, 
we thus have to first isolate the necessary functional capabilities that are common 
to realizing such autonomy for teaming robots.
The aim of the article is to do
just that and thus provide a framework that can serve as the basis for
the development of cognitive robotic teammates.



==> sections/overview.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Transitioning to a Cognitive Teaming Agent} % (fold)
\label{sec:new_view}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figure/agent}
\caption{Traditional view of the goal-based intelligent agent architecture \cite{russell_artificial_2010} that describes how the agent models the world, senses changes in the environment, plans to achieve goals and acts to execute the plans.}
\label{fig:agent}
\end{figure}

In this section, we characterize how each step in the 
``{\it Sense-Model-Plan-Act}'' (SMPA) cycle of the classical goal-based agent view \cite{russell_artificial_2010} (shown in Fig.~\ref{fig:agent}) 
has to be updated to facilitate the mental modeling of the human in the loop 
in order to enable a truly cognitive teaming agent (shown in Fig.~\ref{fig:newagent}).
Specifically, we introduce the Human Mental Model (HuMM) as a key 
in the robot's deliberative process.

%The mental modeling of the other agents (in particular humans in this case) changes the view of an agent. 
%In this section, we start with a typical view of a goal-based agent as depicted in
%Fig.~\ref{fig:agent} and consider the extensions that have to be made
%to this classical agent view \cite{russell_artificial_2010} to enable a cognitive teaming agent to support the various capabilities we have described earlier.  
%In particular, our objective is to characterize how each step in the 
%``{\it Sense-Model-Plan-Act}'' (SMPA) cycle of a typical goal-based
%agent will change for a cognitive teaming agents.
%Next, we provide an overview of the new aspects of this ``{\it Sense-Model-Plan-Act}''HMM cycle, focusing on the changes that must be brought into each functionality:

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figure/newagent}
\caption{An updated view of the architecture of a cognitive teaming agent acknowledging the need to account for the human's mental state by means of what we refer to as \textbf{Hu}man \textbf{M}ental \textbf{M}odeling or HuMM.}
\label{fig:newagent}
\end{figure}

\vspace{5pt}
\paragraph{\textbf{Sense}} The robotic agent can no longer sense passively to
  check that the preconditions of an action are satisfied, or after it
  applies an action to the world to confirm that it is updated
  accordingly (``what the world is like now'' in
  Fig.~\ref{fig:agent}).  In teaming scenarios, the robotic agent
  needs to proactively make complex sensing plans that interact
  closely with other functionalities (i.e., {\it Model} and {\it
    Plan}) to maintain a proper mental state (such as intentions,
  knowledge and beliefs) of its human teammates in order to infer
  about their needs.  For example, how the robot should behave is
  dependent on how much and what type of help the human requires,
  which in turn depends on the observations about the human teammates
  such as their behavior and workload.  Furthermore, the inference
  about the human mental state should be informed by the human model
  that the robot maintains about the human's
  capabilities and preferences.  For example, if a human teammate does
  not drink coffee, the robot should probably consider tea instead
  when asked to fetch a drink.  
  Note that directly asking humans (i.e., explicit communication) 
  should also be considered as a specific form of sensing.
  
\vspace{5pt}
\paragraph{\textbf{Model}} Correspondingly, ``what the world is like now''
  needs to include not only environmental states, but also mental
  states of the team members (including humans and maybe even other
  robots under certain situations).  Hence, we need an augmented state
  model that can also represent the mental, in addition to the
  physiological (e.g., human temperature, levels of exhaustion, bodily
  stress, and remaining energy) and physical states of human teammates
  (e.g., maximum running speed, and lifting strength).  Here, mental
  states may not only include cognitive and affective states such as
  the human's task-relevant beliefs, goals, preferences, and
  intentions, but also, more generally, emotions, workload,
  expectations, trust and etc.  ``What my actions do to the world'' then
  needs to include the effects of the robot's actions on the team
  member's mental state, in addition to the effects on their
  physiological and physical states and the observable environment;
  ``How the world evolves'' now also requires rules that govern the
  evolution of agent mental states based on their interactions with
  the world (including information exchange through communication);
  ``What it will be like'' will thus be an updated state presentation
  that not only captures the world state, agent physiological and
  physical state changes based on their actions and current states,
  but also those mental state changes caused by the agent itself and
  other team members.
	
\vspace{5pt}
\paragraph{\textbf{Plan}} ``What action I should do'' now involves more
  complex decision-making that must also consider human mental state.
  Furthermore, since the robot actions now can influence not only the
  state of the world but also the mental state of the humans, the
  planning process must also consider how the actions may influence
  their mental state and even how to manipulate such mental state.
  For example, in teaming scenarios, it is important to maintain a
  shared mental state between the teammates.  This requires the robots
  to generate behavior that is expected and predictable to the human
  teammates such that the humans would be able to understand the robot
  intention.  On the other hand, a shared mental state does not
  necessarily mean that every piece of information needs to be
  synchronized.  Given the limitation on human cognitive load, sharing
  only necessary information is more practical between different
  teammates working on different parts of the team task.  A properly
  maintained shared mental state between the teammates can contribute
  significantly to the efficiency of teaming since it can reduce the
  necessity of explicit communication in many situations.

\vspace{5pt}
\paragraph{\textbf{Act}} In addition to physical actions, we now also have
  communication actions that can change the mental state of the humans
  by changing their beliefs, intents, etc.  Actions to affect the human's 
  mental state do not have to be linguistic (direct);
  stigmergic actions to instrument the environment 
  can also inform the humans such that
  their mental states can be changed.  Given that an action plan is
  eventually realized via the activation of effectors by providing
  motor commands, {\it Act} must be tightly integrated with {\it
    Plan}.  While {\it Plan} generates the sequence of actions to be
  realized, motor commands can create different motion trajectories to
  implement each action and can in turn impact how the plan would be
  interpreted since different realizations can exert different
  influences on the human's mental states based on the context.
  Hence, it is important to carefully choose the motor commands so
  that the trajectories are ``legible'' to the humans for them to
  understand the behaviors of the robot at the motion level.

\vspace{5pt}
\paragraph{\textbf{Remark}} 
Changes to ``model'' in Figure \ref{fig:newagent} is a direct result of the requirement of human mental modeling.  
Coarsely speaking, changes to ``sense'' contribute to the recognition of teaming context,
changes to ``plan'' contribute to the anticipation of team behavior and ``act'',
and changes to ``act'' contribute to the determination of proper actions at both the action and motion levels.
In practice, these four functionalities are tightly integrated in the behavior loop.

